Rethinking Softmax with Cross-Entropy: Neural Network Classifier as Mutual Information Estimator

Mutual information is widely applied to learn latent representations of observations, whilst its implication in classification neural networks remain to be better explained. We show that optimising the parameters of classification neural networks with softmax cross-entropy is equivalent to maximising the mutual information between inputs and labels under the balanced data assumption. Through experiments on synthetic and real datasets, we show that softmax cross-entropy can estimate mutual information approximately. When applied to image classification, this relation helps approximate the point-wise mutual information between an input image and a label without modifying the network structure. To this end, we propose infoCAM, informative class activation map, which highlights regions of the input image that are the most relevant to a given label based on differences in information. The activation map helps localise the target object in an input image. Through experiments on the semi-supervised object localisation task with two real-world datasets, we evaluate the effectiveness of our information-theoretic approach.

==> secs/abs_old.tex <==
The cross-entropy loss with the softmax output is a standard choice to train a neural network classifier. While it is reasonable to reduce the cross-entropy between outputs of a neural network and labels, the implication of cross-entropy with softmax on the relation between inputs and labels remains to be better explained. We show that training a neural network with cross-entropy maximises the mutual information between inputs and labels through a variational form of the mutual information. The result provides an alternative view of the neural network classifier as a mutual information estimator. This leads us to develop an informative class activation map (infoCAM) that locates the most informative features of input toward a label given a classification task. When applied to an image classification task, infoCAM performs better than the traditional class activation map in the weakly supervised object localisation task.

%One common approach to train a neural network classifier consists of two steps. First, to normalise the outputs to be between 0 and 1. Second, to calculate cross-entropy by viewing the normalised values as probabilities. This approach is popular for training neural network classifiers. However, we argue that viewing the normalised values as probabilities is artificial. Thus, the cross-entropy-based view of neural network classifiers lacks natural coherence. To reduce the artificial interpretation of neural network classifiers, we propose an alternative view. We view neural network classifiers as mutual information estimators. Consequently, training becomes maximising the mutual information between inputs and labels. Moreover, viewing neural network classifiers as mutual information estimators is not only better from the theoretical perspective. The new view can also contribute to practical applications. We present two examples. First, to improve the classification accuracy. Second, to localise the objects about given labels within images. Extensive experimental results support the practical benefits of the new information-theoretic view of neural network classifiers as mutual information estimators.


\begin{comment}
One common approach of training a neural network includes two steps: first, to normalise the outputs to be between 0 and 1; second, to calculate cross-entropy by viewing the normalised values as probabilities. Despite the popularity of this training approach, we argue that viewing the normalised values as probabilities is artificial, making the view of training neural network classifiers lack coherence. To this end, we propose an alternative view of neural network classifiers as mutual information evaluators: training is to maximise the mutual information between inputs and labels. Moreover, our new view is not only more theoretically coherent, but it can also contribute to practical applications. We present two examples: to improve the classification accuracy, in particular when the datasets are imbalanced, and to localise the relevant objects within an image about given labels, with either single or multiple objects within an image. Extensive experimental results support the practical excellence of the new information-theoretic view of neural network classifiers as mutual information evaluators. 
\end{comment}
\begin{comment}
The practical excellence of the new information-theoretic view has been

One common approach of training a neural network classifier is to first normalise the outputs to be between 0 and 1, followed by viewing the normalised values as probabilities for 


Despite the pervasiveness of utilising cross-entropy as loss functions for neural network classifiers, we argue this view can be artificial since it requires interpreting the normalised outputs as probabilities. To make the view of neural network classifiers more rationale, 

interpreting the normalised outputs as probabilities

the seemingly pervasive application of information theory in neural network classifiers, we argue interpreting the normalised outputs as probabilities for further calculating cross-entropy can be artificial, making neural network classifiers lack coherence. In this paper, with the aid of variational inference, we propose an alternative view of neural network classifiers as mutual information evaluators, without modifying the network structures. Through experiments on synthetic datasets, we show neural network classifiers can estimate mutual information accurately. 
\end{comment}
\begin{comment}
Mutual information is widely applied to learn latent representations of observations, whilst its implication in classification neural networks remain to be better explained. We show that optimising the parameters of classification neural networks with softmax cross-entropy is equivalent to maximising the mutual information between inputs and labels under the balanced data assumption. Through experiments on synthetic and real datasets, we show that softmax cross-entropy can estimate mutual information approximately.
When applied to image classification, this relation helps approximate the point-wise mutual information between an input image and a label without modifying the network structure. To this end, we propose infoCAM, informative class activation map, which highlights regions of the input image that are the most relevant to a given label based on differences in information. The activation map helps localise the target object in an input image. Through experiments on the semi-supervised object localisation task with two real-world datasets, we evaluate the effectiveness of our information-theoretic approach.
\end{comment}

==> secs/intro_old.tex <==
\section{Introduction}
% Neural network classifiers are important 
% It has two consequences. 
Neural network classifiers play an essential role in artificial neural networks~\cite{abiodun2018state}. First, they can solve long-term challenges that are hard for traditional approaches~\cite{lecun2006tutorial}. For example, image classification has been a challenging problem, however, neural network classifiers' performance surpasses other traditional approaches by a large margin~\cite{krizhevsky2012imagenet}. Also, neural network classifiers can contribute to training models for object detection~\cite{he2017mask}. 
\begin{comment}
Also, neural network classifiers can contribute to training generative adversarial networks. Specifically, a generative adversarial network uses a neural network classifier to discern whether an image is generated or not. Therefore, the quality of the neural network classifier decides the performance of the generated images. 
\end{comment}

\begin{comment}
Second, apart from classification, they can contribute to other learning tasks. We illustrate examples. First, image classification has been a challenging problem. However, neural network classifiers made breakthroughs. Their performance surpasses other traditional approaches with a large margin. 

Neural network classifiers play an essential role in the study of artificial neural networks~\cite{abiodun2018state}: not only can they solve important challenges with which traditional approaches have long-term difficulties~\cite{lecun2006tutorial}, but their breakthroughs can also promote other learning tasks. As illustrations: to the former, a neural network named AlexNet makes significant progress toward this problem by surpassing other traditional approaches with a large margin in 2012, leading the current boom of deep learning~\cite{krizhevsky2012imagenet}; to the latter, training a pleasing generative adversarial network, a modern unsupervised learning model, depend on the quality of the internal neural network classifier to discern the genuineness of the given data~\cite{goodfellow2014generative}.  
\end{comment}

% Why information theory for neural networks 
Information theory has been long employed to study neural network classifiers~\cite{gish1990probabilistic}. For example, cross-entropy is a term from information theory. It is almost the canonical loss function for neural network classifiers~\cite{pang2019rethinking}. Using information theory to study neural network classifiers is intuitive and plausible. We justify as follows. Neural network classifiers process complex and dimensional information to classify the given data to certain classes. To quantify the amount of information that is processed by neural network classifiers, we can resort to information theory, since information theory is a principled framework for measuring how much information one can obtain from data~\cite{belghazi2018mutual}. 

% Current problems of connecting NNs with information theory
It is popular and widely-accepted to study and optimise neural network classifiers from information-theoretic perspectives. However, we argue that current connections between neural network classifiers and information theory lack coherence. We justify as follows. To obtain cross-entropy for training a neural network classifier, we need to convert the outputs to be within the range between 0 and 1. We conduct the normalisation with a sigmoid or softmax~\cite{goodfellow2016deep}. Afterwards, it is popular to interpret the normalised values as probabilities, since they are smaller than one. Nevertheless, these 'artificially' normalised outputs are not consistent with the definition of probability. To explain, if one changes the normalisation function from one to the other, the normalised values vary accordingly. However, from the perspective of the law of large numbers, probabilities are inherent properties so they should be constant. 
\begin{comment}
Despite the pervasiveness and popularity of defining and analysing neural network classifiers from information-theoretic perspectives, we argue current connections between neural network classifiers and information theory may lack coherence. We justify this argument as follows: one imperative step for evaluating cross-entropy of a neural network classifier is to convert the outputs to be within the range between 0 and 1, using normalisation functions such as sigmoid or softmax~\cite{goodfellow2016deep}. The converted results are commonly interpreted as probabilities since they are non-negative and smaller than one. However, these artificially normalised outputs are not consistent with the definition of probability: the normalised values vary in response to changing normalisation methods, whilst from the perspective of the law of large numbers, probabilities are inherent properties so they should be of constancy. 
\end{comment}

% New view 
In sum, it is popular to use cross-entropy as the loss function to train neural network classifiers. However, in order to use cross-entropy, we need to interpret (or assume) the normalised outputs of neural network classifiers as probabilities, and the interpretation seems to be artificial. Thus, we seek an alternative information-theoretic view of neural network classifiers that is more coherent. That is, the new view contains less artificial assumptions. To this end, we propose viewing neural network classifiers as mutual information evaluators: using a variational form of mutual information to prevent interpreting outputs as probabilities. 
\begin{comment}
In sum, using cross-entropy as the loss function to train neural network classifiers requires interpreting normalised values as probabilities; such interpretation, however, seem to be artificial. Thus, we seek for an alternative information-theoretic view of neural network classifiers that is more coherent, \ie, less artificial interpretations. To this end, we propose viewing neural network classifiers as mutual information evaluators: using a variational form of mutual information to prevent interpreting outputs as probabilities. 
\end{comment}

% The advantage of the new view
We propose to view neural network classifiers as mutual information evaluators. This new information-theoretic view is not only better from the theoretical perspective, but can also contribute to practical applications. We exhibit two in this paper. First, to improve classification accuracy. Instead of using cross-entropy as loss functions, we can use mutual information can improve the performance of neural network classifiers. Second, to more precisely locate within images the objects which are labels overall. We decompose the overall pointwise mutual information into the sum of sub-regions of an image, and identify the ones with high decomposed mutual information. 
\begin{comment}
The new information-theoretic view of neural network classifiers can not only be more plausible in theory, but it can also help to optimise the application neural network classifiers in various practical tasks via considering the outputs as the mutual information between the inputs and the labels. We demonstrate two applications in this paper: improving classification accuracy and locating the objects relating to the labels of an image more precisely. The former is due to modifying loss functions to make the opposite of loss become mutual information and the latter receives motivation from building the mathematical relationship between the mutual information of the entire image and its sub-regions. 
\end{comment}

In summary we outline our contributions in the corresponding sections as follows: 
\begin{itemize}
    \item We show how to convert a neural network classifier into a mutual information evaluator. We also empirically show that the converted mutual information evaluator can accurately estimate mutual information. 
    \item We show mutual information evaluators can perform classification more accurately than traditional neural network classifiers. When the dataset is imbalanced, the evaluators outperform the state-of-the-art classifier. 
    \item We show how viewing neural network classifiers as mutual information evaluators can help to locate the most relevant regions of images about certain labels. We achieve a new state-of-the-art result on Tiny-ImageNet.
\end{itemize}

\begin{comment}
In summary, we outline our contributions in the corresponding sections as follows: 
\begin{itemize}
    \item In \autoref{sec:conn}, we prove that classification neural networks that optimise their weights to minimise softmax cross-entropy are equivalent to those that maximise mutual information between inputs and labels with a balanced dataset.
    \item In \autoref{sec:mi_class_exp}, we empirically evaluate the effectiveness of classification mutual information estimators via synthetic and real-world datasets.
    \item In \autoref{sec:cam}, we propose infoCAM. A map that reveals the most relevant regions of an image with respect to the target label based on the difference of mutual information.
    \item In \autoref{sec:exp}, we demonstrate the performance of the infoCAM on WSOL results, achieving a new state-of-the-art result on Tiny-ImageNet.
\end{itemize}
\end{comment}

\begin{comment}
using a variational form of mutual information instead of interpreting outputs as probabilities. 

It is intuitive and plausible to study neural network classifiers with information theory: neural network classifiers are designed to process complex and multidimensional information in order to classify the given data to certain classes, and information theory provides a principled framework for quantifying the information that has been processed by neural networks. Despite various information-theoretic terms have been employed 


For example, to the former, image classification has been a long-lasting challenge since the inception of computer vision, as successful recognition of objects lays the key foundation for endless down-stream applications, such as building autonomous cars and developing face IDs. In 2012, a neural network named AlexNet makes significant progress toward this problem by surpassing other traditional approaches with a large margin, leading the current boom of deep learning~\cite{krizhevsky2012imagenet,lecun2015deep}. 

and surpasses by a large margin all the traditional approaches at the time~\cite{krizhevsky2012imagenet,lecun2015deep}.

It is intuitive and plausible to study neural networks with information theory: both natural and artificial neural networks are evolved or designed to process complex and multidimensional information, and information theory provides a principled framework for quantifying the information that has been processed by neural networks. 

\section{Introduction}

%(The importance of classification neural networks) 
In 2012, AlexNet makes significant progress toward ILSVRC: the ImageNet Large Scale Visual Recognition Challenge, and surpasses by a large margin all the traditional approaches at the time~\cite{krizhevsky2012imagenet,lecun2015deep}. As a result, such classification neural networks start playing a crucial role in the contemporary machine learning and computer vision community~\cite{lecun2015deep}. Apart from their strong categorisation capability, classification neural networks contribute to other tasks, \eg generative adversarial networks use a classification network for producing  visually-realistic images~\cite{goodfellow2014generative}, and object segmentation networks such as Mask-RCNN use classification networks for object detection~\cite{he2017mask}. 

%(NN uses softmax, which is artificial)
The softmax function, or softmax in short, is the basic building block of the final layer of classification models. Previous studies interpret softmax as a function that transforms non-normalised values to probabilities since the outputs of softmax sum up to one and are non-negative~\cite{bridle1990probabilistic}. Despite the popularity of such an interpretation, softmax under this view seems to be an artificial adjustment to enforce that the outputs of classification neural networks satisfy probability axioms. This raises a question on an alternative view of softmax being more than a transformation function.

%(Connection between NN and MI and its novelty)
In this paper, we present an information-theoretic interpretation of softmax with cross-entropy. With a variational form of mutual information, we formally prove that optimising model parameters with the softmax cross-entropy is equal to maximising the mutual information between input data and labels via assuming uniform distribution of labels. The connection provides an alternative view on the classifier as a mutual information estimator. We further propose a probability-corrected version of softmax which relaxes the uniform distribution condition. Based on experiments with synthetic datasets, we demonstrate the performance of softmax on mutual information estimation.

%(Why it's important: application - infocam)
The connection between classification and information gives a new intuition on interpreting the output of the classifier. As an application, we investigate the image classification problem, especially targeting a class activation map for weakly-supervised object classification tasks. The class activation map aims to find the region which is the most relevant to the target class. We propose a new approach, dubbed as infoCAM, to compute a class activation map based on the point-wise mutual information obtained by classification.
Through the experiments, we evaluate the effectiveness of infoCAM on weakly-supervised object localisation with Tiny-ImageNet~\cite{tiny_imagenet} and CUB-200-2011~\cite{wah2011caltech} datasets.

%(Contribution)
In summary, we outline our contributions in the corresponding sections as follows: 
\begin{itemize}
    \item In \autoref{sec:conn}, we prove that classification neural networks that optimise their weights to minimise softmax cross-entropy are equivalent to those that maximise mutual information between inputs and labels with a balanced dataset.
    \item In \autoref{sec:mi_class_exp}, we empirically evaluate the effectiveness of classification mutual information estimators via synthetic and real-world datasets.
    \item In \autoref{sec:cam}, we propose infoCAM. A map that reveals the most relevant regions of an image with respect to the target label based on the difference of mutual information.
    \item In \autoref{sec:exp}, we demonstrate the performance of the infoCAM on WSOL results, achieving a new state-of-the-art result on Tiny-ImageNet.
\end{itemize}
\end{comment}

% Neural network classifiers are important 
%Neural network classifiers play an essential role in artificial neural networks~\cite{abiodun2018state}. First, they can solve long-term challenges that are hard for traditional approaches~\cite{lecun2006tutorial}. For example, image classification has been a challenging problem, however, neural network classifiers' performance surpasses other traditional approaches by a large margin~\cite{krizhevsky2012imagenet}. Also, neural network classifiers can contribute to training models for object detection~\cite{he2017mask}. 

% Why information theory for neural networks 
%Information theory has been long employed to study neural network classifiers~\cite{gish1990probabilistic}. For example, cross-entropy is a canonical loss function for modern neural network classifiers~\cite{pang2019rethinking}. Using information theory to study neural network classifiers is intuitive and plausible. We justify as follows. Neural network classifiers process complex and dimensional information to classify the given data to certain classes. To quantify the amount of information that is processed by neural network classifiers, we can resort to information theory, since information theory is a principled framework for measuring how much information one can obtain from data~\cite{belghazi2018mutual}. 

% Current problems of connecting NNs with information theory
% However, we argue that current connections between neural network classifiers and information theory lack coherence. As previously stated, it is popular to use cross-entropy to view how neural network classifiers perform from an information-theoretic perspective. However, cross-entropy only reflects the relationship between the outputs of the neural network classifier and the ground-truth labels. We are also interested in the information-theoretic relationship between the inputs and the labels. 

%In sum, it is popular to use cross-entropy to train or to understand neural network classifiers. However, proper interpretation between the inputs of the neural network and the ground truth labels can not be well understood by the cross-entropy. Thus, we seek an alternative information-theoretic view of neural network classifiers that is more coherent. That is, the new view can reflect the information-theoretic relationship between the inputs and the labels. Interestingly, we discover that with just minor modification on the sigmoid or softmax functions, the training objective becomes mutual information maximisation. To be more specific, using the modified sigmoid or softmax, training neural network classifiers is to maximise the mutual information between the inputs and the labels. 

%The new information-theoretic view of neural network classifiers allow us to directly access the most informative region of an image with respect to the labels. Consequently, we can locate the most relevant toward the labels within an image. Thus, we propose the informative class activation map (infoCAM). Compared to the traditional class activation map, infoCAM exhibits better performance in the weakly supervised object localisation task. Furthermore, it brings an information-theoretic interpretation to class activation maps. 

% In summary, we outline our contributions as follows: 
% \begin{itemize}
%     \item The previous information-theoretic view, based on cross-entropy, only reflects the relationship between the outputs and the labels. We show that with minor modifications on sigmoid or softmax, neural network classifiers then become mutual information estimators. As a result, mutual information estimators exhibit the information-theoretic relationship between the inputs and the labels. 
%     \item We empirically demonstrate that our mutual information estimators can accurately evaluate mutual information. We also show mutual information estimators can perform classification more accurately than traditional neural network classifiers. When the dataset is imbalanced, the estimators outperform the state-of-the-art classifier. 
%     \item Mutual information estimators allow us to directly access the most informative regions toward the labels within an image. Thereby, we propose the informative class activation map (infoCAM). For the weakly supervised object localisation task, we achieve a new state-of-the-art result on Tiny-ImageNet with infoCAM. 
% \end{itemize}


%%% From the previous intro
%(The importance of classification neural networks) 
% Neural network classifiers play an important role in the contemporary machine learning and computer vision~\cite{lecun2015deep} since the emergence of AlexNet~\cite{krizhevsky2012imagenet}. Often, the softmax function is used as a basic building block of the final layer of classification models. Previous studies interpret softmax as a function that transforms non-normalised values to probabilities since the outputs of softmax sum up to one and are non-negative~\cite{bridle1990probabilistic}. Despite the popularity of such an interpretation, softmax under this view seems to be an artificial adjustment to enforce that the outputs of classification neural networks satisfy probability axioms. This raises a question on an alternative view of softmax being more than a transformation function.

% %(Connection between NN and MI and its novelty)
% In this paper, we present an information-theoretic interpretation of softmax with cross-entropy. With a variational form of mutual information, we formally prove that optimising model parameters with the softmax cross-entropy is equal to maximising the mutual information between input data and labels via assuming uniform distribution of labels. The connection provides an alternative view on the classifier as a mutual information estimator. We further propose a probability-corrected version of softmax which relaxes the uniform distribution condition. Based on experiments with synthetic datasets, we demonstrate the performance of softmax on mutual information estimation.

% %(Why it's important: application - infocam)
% The connection between classification and information gives a new intuition on interpreting the output of the classifier. As an application, we investigate the image classification problem, especially targeting a class activation map for weakly-supervised object classification tasks. The class activation map aims to find the region which is the most relevant to the target class. We propose a new approach, dubbed as infoCAM, to compute a class activation map based on the point-wise mutual information obtained by classification.
% Through the experiments, we evaluate the effectiveness of infoCAM on weakly-supervised object localisation with Tiny-ImageNet~\cite{tiny_imagenet} and CUB-200-2011~\cite{wah2011caltech} datasets.

% %(Contribution)
% In summary, we outline our contributions in the corresponding sections as follows: 
% \begin{itemize}
%     \item In \autoref{sec:conn}, we prove that classification neural networks that optimise their weights to minimise softmax cross-entropy are equivalent to those that maximise mutual information between inputs and labels with a balanced dataset.
%     \item In \autoref{sec:mi_class_exp}, we empirically evaluate the effectiveness of classification mutual information estimators via synthetic and real-world datasets.
%     \item In \autoref{sec:cam}, we propose infoCAM. A map that reveals the most relevant regions of an image with respect to the target label based on the difference of mutual information.
%     \item In \autoref{sec:exp}, we demonstrate the performance of the infoCAM on WSOL results, achieving a new state-of-the-art result on Tiny-ImageNet.
% \end{itemize}


==> secs/preli_old.tex <==
\section{Preliminaries}
\label{sec:pre}
In this section, we first define the notations used throughout this paper. We then introduce the definition of mutual information and variational forms of mutual information. 

\subsection{Notation}
%We provide notation in the first place in the interest of precise and concise expressions. 
We let training data consisting of $M$ classes and $N$ labelled instances as $\{ (\mathbf{x}_{i}, y_{i}) \}_{i=1}^{N}$, where $y_i \in \mathcal{Y} = \{ 1, ... , M \}$ %\remove{of each datum $(\mathbf{x}_n, y_n)$} 
is a class label of the input $\mathbf{x}_i$. We let $n_{\mathbf{\phi}}(\mathbf{x}): \mathcal{X} \rightarrow \mathbb{R}^M$ be a neural network parameterised by $\phi$, where $\mathcal{X}$ is a space of input $\mathbf{x}$. Without additional clarification, we assume $\mathcal{X}$ to be a compact subset of $D$-dimensional Euclidean space. 
%Neural network $n_{\mathbf{\phi}}(\mathbf{x_n})$ maps input $\mathbf{x}$ to an output vector $\mathbf{z_n} \in \mathbb{R}^{M}$, and possess tunable parameter $\mathbf{\phi}$. 
%We use $[n_{\mathbf{\phi}}(\mathbf{x})]_y$ to denote the $y$-th element of an output for neural network $n_{\mathbf{\phi}}$ with input $\mathbf{x}$.
We denote by $P_{XY}$ some joint distribution over $\mathcal{X} \times \mathcal{Y}$, with $(\mathbf{X}, Y) \sim P_{XY}$ a pair of random variables. $P_{X}$ and $P_{Y}$ are the marginal distributions of $\mathbf{X}$ and $Y$, respectively. We remove a subscript from the distribution if it is clear from context.

\subsection{Variational Bounds of Mutual Information}
%\subsubsection{Mutual Information}
%Mutual information evaluates the relationship between two random variables in information theory. 
Mutual information evaluates the mutual dependence between two random variables. 
The mutual information between $\mathbf{X}$ and $Y$ can be expressed as:
\begin{equation}
\label{eq:orig_mi_def}
\mathbb{I}(\mathbf{X}, Y) = \int_{\mathbf{x} \in \mathcal{X}} \bigg[ \sum_{y \in \mathcal{Y}} P(\mathbf{x}, y) \log \big( \frac{P(\mathbf{x}, y)}{P(\mathbf{x}) P(y)} \big) \bigg] d\mathbf{x}. 
\end{equation}

Equivalently, following~\cite{poole2019variational} we may express the definition of mutual information in \autoref{eq:orig_mi_def} as:
\begin{equation}
\label{eq:cond_mi_def}
\mathbb{I}(\mathbf{X}, Y) = \mathbb{E}_{(\mathbf{X}, Y)} \bigg[ \log \frac{P(y | \mathbf{x})}{P(y)} \bigg],
\end{equation}
where $\mathbb{E}_{(\X, Y)}$ is the abbreviations of $\mathbb{E}_{(\X, Y) \sim P_{XY}}$. 
Computing mutual information directly from the definition is, in general, intractable due to integration. %We therefore derive its variational lower bound to make it tractable. 

%\subsubsection{Barber-Agakov (BA) Representation}
% \label{subsec:ba_rep}
\textbf{Variational form}: Barber and Agakov introduce a commonly used lower bound of mutual information via a variational distribution $Q$~\cite{barber2003algorithm}, derived as:
\begin{align}
\label{eq:ba_def}
\mathbb{I}(\mathbf{X}, Y) &= \mathbb{E}_{(\X, Y)} \bigg[ \log \frac{P(y | \mathbf{x})}{P(y)} \bigg] \notag \\
&= \mathbb{E}_{(\X, Y)} \bigg[ \log \frac{Q(y | \mathbf{x})}{P(y)} \frac{P(y | \mathbf{x})}{Q(y | \mathbf{x})} \bigg] \notag \\
&= \mathbb{E}_{(\X, Y)} \bigg[ \log \frac{Q(y | \mathbf{x})}{P(y)}
\bigg] + 
\underbrace{\mathbb{E}_{(\X, Y)} \bigg[ \log \frac{P(\mathbf{x},y)}{Q(\mathbf{x},y)} \bigg]}_{D_{KL}(P(\mathbf{x}, y) || Q(\mathbf{x}, y))} \notag - 
\underbrace{\mathbb{E}_{(\X)} \bigg[ \log \frac{P(\mathbf{x})}{Q(\mathbf{x})} \bigg]}_{D_{KL}(P(\mathbf{x}) || Q(\mathbf{x}))} \notag \\
&\ge \mathbb{E}_{(\X, Y)} \bigg[ \log \frac{Q(\mathbf{x},y)}{P(\x)P(y)} \bigg]. 
\end{align}
The inequality in \autoref{eq:ba_def} holds since KL divergence maintains non-negativity. This lower bound is tight when variational distribution $Q(\mathbf{x},y)$ converges to joint distribution $P(\mathbf{x},y)$, i.e., $Q(\mathbf{x},y) = P(\mathbf{x},y)$.

The form in \autoref{eq:ba_def} is, however, still hard to compute since it is not easy to make a tractable and flexible variational distribution $Q(\mathbf{x},y)$. Variational distribution $Q(\mathbf{x},y)$ can be considered as a constrained function which has to satisfy the probability axioms. Especially, the constraint is challenging to model with a function estimator such as a neural network. To relax the function constraint, McAllester \etal \cite{mcallester2018formal} further apply reparameterisation and define $Q(\mathbf{x},y)$ in terms of an unconstrained function $f_{\phi}$ parameterised by $\phi$ as:
\begin{equation}
\label{eq:repara_q}
Q(\mathbf{x},y) = \frac{P(\x)P(y)}{E_{y' \sim P_Y}[ \exp(f_{\mathbf{\phi}}(\mathbf{x}, y')) ]} \exp(f_{\mathbf{\phi}}(\mathbf{x}, y)).
\end{equation}
As a consequence, the variational lower bound of mutual information $\mathbb{I}(\mathbf{X}, Y)$ can be rewritten with function $f_{\mathbf{\phi}}$ as:
\begin{align}
\label{eq:mi_f_low_bound}
\mathbb{I}(\X, Y) \ge \mathbb{E}_{(\X, Y)} \bigg[ \log \frac{\exp(f_{\mathbf{\phi}}(\mathbf{x}, y))}{ E_{y'}[ \exp(f_{\mathbf{\phi}}(\mathbf{x}, y')) ]}  \bigg].
\end{align}
One can estimate mutual information without any constraint on $f$.
%where $f_{\mathbf{\phi}}$ is modelled by any neural network thanks to the removal of the function constraint~\cite{mcallester2018formal}. 
Through the reparameterisation, the MI estimation can be recast as an optimisation problem.


==> secs/temporary.tex <==
\section{Temporary}

Remember that one of our goal is to find the most representative patch from an image which is highly informative to identify the label of the image. The point-wise mutual information between input image patch $X_i$ and the label $Y$ would be highly appreciated to solve such problem.

Let $X$ can be decomposed into multiple features $X = \{X_1, X_2, ..., X_R\}$, the mutual information between $X$ and $Y$ can be rewritten as
\begin{align}
    MI(X,Y) &= \mathbb{E}_{(X,Y)}\bigg[ \log \frac{P(X|Y)}{P(X)} \bigg]  \\
            &= \mathbb{E}_{(X,Y)}\bigg[ \log \frac{P(X_1,..,X_R|Y)}{P(X_1,...,X_R)} \bigg] \notag \\
            &= \mathbb{E}_{(X,Y)}\bigg[ \log \frac{P(X_i|X_{-i}, Y)}{P(X_i|X_{-i})} \bigg] \hfill \text{(by chain-rule)} \notag \\
            &\geq \mathbb{E}_{(X,Y)}\bigg[ \log \frac{f(X_i, X_{-i}, Y)}{\mathbb{E}_{(X_{-i}',Y')}[f(X_i, X_{-i}', Y')]} \bigg] \quad \notag\\
            &\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\text{(By \autoref{eq:mi_f_low_bound})} \notag,
            % I donno why \hfill doesn't work
\end{align}
where $f$ is a function that maps $\mathcal{X}_i \times \mathcal{X}_i^{R-1} \times \mathcal{Y} \rightarrow \mathbb{R}$.

Note that function $f$ should be permutation invariant to make the order of $X_i$ irrelevant. Let $\Pi_R$ be the set of all permutations of indices ${1,...,R}$. A function $f$ is permutation invariant iff $f(X) = f(\pi(X))$, $\forall \pi \in \Pi_R$ \cite{zaheer2017deep}. An example of such function is:
\begin{align}
    f(\{x_1,...,x_R\}) = \sigma(\text{pool}(\{\phi(x_1),...,\phi(x_R)\})),
\end{align}
where pool is a pooling operation, $\phi$ is learnable function, and $\sigma$ is a non-linear activation function.

We can learn a neural network $f:X^R \rightarrow \mathbb{R}^{|\mathcal{Y}|}$ with the following objective:
\begin{align}
    L =\mathbb{E}_{(X,Y)}\Big[& \log f(X_i, X_{-i}, Y)  \notag\\
     &- \log \mathbb{E}_{(X_{-i}',Y')}\big[f(X_i, X_{-i}', Y')\big] \Big].
\end{align}
Note that in its maximum, we can obtain a point-wise mutual information between $X_i$ and $Y$.
The empirical loss function will be
\begin{align}
    L =\sum_{(x^{n},y^{n}) \in \mathcal{D}}\Big[& \log f(x_i^n, x_{-i}^n, y^n)  \notag\\
     &- \log \big[f(x_i, x_{-i}', y')\big] \Big],
\end{align}
where we take a randomly sample of $x_{-i}'$ and $y'$ from an empirical distribution.

For some applications such as image modelling, $x_i$ can be considered as a patch of image $x_i$. Image patches, however, should not be modelled by permutation invariant functions, because adjacency structure between patches are important factor to model the image. To model such structured data, we can place non-invariant neural network blocks before $f$. For example, the output of CNN is a set of image features which is modelled via permutation invariant function. Therefore, we can construct an end-to-end learning model by replacing an input of $f$ through CNN layers
\begin{align}
    L =\sum_{(x^{n},y^{n}) \in \mathcal{D}}\Big[& \log f([g(x^n)]_i, [g(x^n)]_{-i}, y^n) \\
     & -\log \big[f([g(x^n)]_i, [g(x')]_{-i}, y')\big] \Big], \notag
\end{align}
where $g$ is a set of layers taking $x\in\mathcal{X}$ as an input, and, with a slight abuse of notation, we let $[\cdot]_i$ and $[\cdot]_{-i}$ is a selector operation used to represent $i$th output and the output except $i$th component inside the brackets, respectively.

\subsection{PMI with Embedded Classifier}
We explicitly model $f(x_i, x_{-i}, y) = [n_\phi(x, x_{-i})]_{y}$.

\subsection{Experiments}
We need two experiments. First, WSOL. Second, classification via $f$. WSOL needs to achieve SOTA. WSOL task is slightly different from info-CAM, because we can directly compute the PMI from the objective. The classification needs to show reasonable performance. Therefore, we can use interpretable model without losing too much classification performance. However, it would be the best if the classification performance is good as well.


